Norm-Resolvent Convergence in Perforated Domains

For several different boundary conditions (Dirichlet, Neumann, Robin), we prove norm-resolvent convergence for the operator $-\Delta$ in the perforated domain $\Omega\setminus \bigcup_{ i\in 2\varepsilon\mathbb Z^d }B_{a_\varepsilon}(i),$ $a_\varepsilon\ll\varepsilon,$ to the limit operator $-\Delta+\mu_{\iota}$ on $L^2(\Omega)$, where $\mu_\iota\in\mathbb C$ is a constant depending on the choice of boundary conditions. This is an improvement of previous results [Cioranescu & Murat. A Strange Term Coming From Nowhere, Progress in Nonlinear Differential Equations and Their Applications, 31, (1997)], [S. Kaizu. The Robin Problems on Domains with Many Tiny Holes. Pro c. Japan Acad., 61, Ser. A (1985)], which show strong resolvent convergence. In particular, our result implies Hausdorff convergence of the spectrum of the resolvent for the perforated domain problem.

==> BoundedPerfDom.tex <==
%\documentclass[11pt,a4paper]{article} 
%
%\usepackage{etex}
%\usepackage[english]{babel}
%\usepackage{tikz}
%\usepackage{pgfplots}
%\usetikzlibrary{fadings,fpu,arrows,decorations.pathmorphing,backgrounds,positioning,fit,petri,patterns}
%\usepackage[utf8]{inputenc}
%\usepackage{graphicx}
%\usepackage[colorlinks=true,linkcolor=black,citecolor=black]{hyperref}
%\usepackage{amsfonts}
%\usepackage{enumerate}
%\usepackage{booktabs}
%\usepackage{array} 
%\usepackage{paralist} 
%\usepackage{subfig} 
%\usepackage{mathtools}
%\usepackage{tabu}
%\usepackage{amsthm}
%\usepackage{empheq}
%\usepackage{amsopn}
%\usepackage{dsfont}
%\usepackage{wrapfig}
%\usepackage[font=small]{caption}
%
%
%\begin{document}
\begin{tikzpicture}[>=stealth,scale=0.8]
	\clip (-0.2,-2.5) rectangle (7.2,2.8);
	\filldraw[fill = gray!20] plot [smooth, tension=0.6] coordinates {(6.5,-1.5) (2,-1.5) (-0.1,0) (2,2) (4,2.5) (5,1.5) (6.7,1) (6.5,-1.5)};
	
	\filldraw[fill = white] (0,0) circle (1mm) ;
		
	\draw (0.7,1.8)node[]{${\Omega_\varepsilon}$} ;
	
	\filldraw[fill = white] (1,0) circle (1mm) ;
	\filldraw[fill = white] (2,0) circle (1mm) ;
	\filldraw[fill = white] (3,0) circle (1mm) ;
	\filldraw[fill = white] (4,0) circle (1mm) ;
	\filldraw[fill = white] (5,0) circle (1mm) ;
	\filldraw[fill = white] (6,0) circle (1mm) ;
	
	\filldraw[fill = white] (1,1) circle (1mm) ;
	\filldraw[fill = white] (2,1) circle (1mm) ;
	\filldraw[fill = white] (3,1) circle (1mm) ;
	\filldraw[fill = white] (4,1) circle (1mm) ;
	\filldraw[fill = white] (5,1) circle (1mm) ;
	\filldraw[fill = white] (6,1) circle (1mm) ;
	
	\filldraw[fill = white] (3,2) circle (1mm) ;
	\filldraw[fill = white] (4,2) circle (1mm) ;
	\draw [black, domain=32.5:-149.5] plot ({0.1*cos(\x)+2},{0.1*sin(\x)+2});
	\filldraw[white] (2,2) circle (0.85mm) ;
%	\draw [black, domain=-20:-123] plot ({0.1*cos(\x)+7},{0.1*sin(\x)+2});
%	\filldraw[white] (7,2) circle (0.92mm) ;
	
	\filldraw[fill = white] (1,-1) circle (1mm) ;
	\filldraw[fill = white] (2,-1) circle (1mm) ;
	\filldraw[fill = white] (3,-1) circle (1mm) ;
	\filldraw[fill = white] (4,-1) circle (1mm) ;
	\filldraw[fill = white] (5,-1) circle (1mm) ;
	\filldraw[fill = white] (6,-1) circle (1mm) ;
%	\draw (6,-1)node[label=east:\Large$\quad\cdots$]{} ;
	
%	\draw [black, domain=6:159] plot ({0.1*cos(\x)+7},{0.1*sin(\x)-3});
%	\filldraw[white] (7,-3) circle (0.92mm) ;
		
%	\draw (1,-1) -- (-0.5,-1) node[anchor=east] {$B_{a_\varepsilon}(i)$};
%	\draw (1,0) -- (-0.5,-1) ;
	
	\draw[->] (0.5,-2) -- (0.89,-2);
	\draw[->] (1.5,-2) -- (1.11,-2);
	\draw[dotted] (0.89,-1) -- (0.89,-2);
	\draw[dotted] (1.11,-1) -- (1.11,-2);
	\draw (1.05,-2.3) node[]{\small${2a_\varepsilon^\iota}$};

	
	\draw[<->] (4.5,-1.9) -- (5.5,-1.9);
%	\draw[->] (5.2,-1.9) -- (5.5,-1.9);
	\draw (5,-2.3) node[]{\small${2\varepsilon}$};
	

	\draw[dotted, shift={(0.5,0.5)}] (-0.7,-2.5) grid (6.7,2.3);
	
%	\draw (-0.7,1.7) -- (0.2,1.9);
%	\draw (0.8,1.8) -- (1.3,1.3);

%	\fill[white] (-3,-3) rectangle (-0.4,-0.4);
	
\end{tikzpicture}
%\end{document}
